A Survey and Benchmark of Automatic Surface Reconstruction from Point Clouds

We present a comprehensive survey and benchmark of both traditional and learning-based methods for surface reconstruction from point clouds. This task is particularly challenging for real-world acquisitions due to factors such as noise, outliers, non-uniform sampling, and missing data. Traditional approaches often simplify the problem by imposing handcrafted priors on either the input point clouds or the resulting surface, a process that can require tedious hyperparameter tuning. In contrast, deep learning models have the capability to directly learn the properties of input point clouds and desired surfaces from data. We study the influence of handcrafted and learned priors on the precision and robustness of surface reconstruction techniques. We evaluate various time-tested and contemporary methods in a standardized manner. When both trained and evaluated on point clouds with identical characteristics, the learning-based models consistently produce higher-quality surfaces compared to their traditional counterparts -- even in scenarios involving novel shape categories. However, traditional methods demonstrate greater resilience to the diverse anomalies commonly found in real-world 3D acquisitions. For the benefit of the research community, we make our code and datasets available, inviting further enhancements to learning-based surface reconstruction. This can be accessed at https://github.com/raphaelsulzer/dsr-benchmark .

==> figures/interpolate_approximate/interpolate_approximate.tex <==
\begin{figure*}
% \captionsetup{justification=centering,font=tiny} % this is for the figure captions
\captionsetup[sub]{labelfont=scriptsize,textfont=scriptsize,justification=centering}
    \centering
    \newcommand{\mywidth}{0.24\textwidth}
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}}
         \subfloat[Open Interpolation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/ifew.jpg}\label{fig:ifew}}
         &  \subfloat[Open Interpolation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/iopen.jpg}\label{fig:iopen}}
         &  \subfloat[Closed Interpolation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/iaclosed.jpg}\label{fig:iclosed}}
        &  \subfloat[Closed Interpolation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/i2closed.jpg}\label{fig:i2closed}}
         
\\  \subfloat[Open Approximation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/afew.jpg}\label{fig:afew}}
        &  \subfloat[Open Approximation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/aopen.jpg}\label{fig:aopen}}         
        &  \subfloat[Closed Approximation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/aclosed.jpg}\label{fig:aclosed}}     
        &  \subfloat[Closed Approximation]{    \includegraphics[width=\mywidth]{figures/interpolate_approximate/a2closed.jpg}\label{fig:a2closed}}  
    \end{tabular}
\caption[Approximating and interpolating surfaces from point clouds]{\textbf{Approximating and interpolating surfaces from point clouds:} A surface generated from point samples can either interpolate (top row) or approximate (bottom row) the samples. Theoretically, there exist an infinite number of surfaces with different geometry and topology that can pass through, or near, the samples. We show eight different surfaces
\protect\tikz[baseline=-.25em] \protect\draw[-, thick, draw = red] (0,0) -- (0.3,0);
reconstructed from the same point cloud
\protect\tikz[baseline=-.35em] \protect\node[circle, draw = none, fill = black, scale = 0.3] {}; \protect\tikz[baseline=-.15em] \protect\node[circle, draw = none, fill = black, scale = 0.3] {}; \protect\tikz[baseline=-.35em] \protect\node[circle, draw = none, fill = black, scale = 0.3] {}; \protect\tikz[baseline=-.15em] \protect\node[circle, draw = none, fill = black, scale = 0.3] {};
in (\subref{fig:ifew}) - (\subref{fig:a2closed}). The point cloud can be seen as a sampling of a part of a real surface.
All reconstructed surfaces are watertight, as they are either closed and boundary-free, or their only boundary is the intersection with the domain boundary \protect\tikz \protect\node [rectangle, thick, draw = blue, minimum width=1, minimum height=0.7] at (0,0) {};.
The surface in (\subref{fig:i2closed}) is non-manifold in the center-vertex. All other surfaces are manifold. Except for  (\subref{fig:a2closed}), all surfaces are comprised of only one component. In contrast to the point cloud depicted here, in our benchmark, we mainly consider point clouds sampled from closed surfaces.
}
    \label{fig:ch2:inter_approx}
\end{figure*}

==> figures/learning_optim/learning_optim.tex <==
\begin{figure*}
% \captionsetup{justification=centering,font=tiny} % this is for the figure captions
\captionsetup[sub]{labelfont=scriptsize,textfont=scriptsize,justification=centering}
    \centering
    \newcommand{\mywidth}{0.13\textwidth}
    \definetrim{mytrim}{50 50 50 50}
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c|@{}c@{}}
        %  &
        %  &
        %  & \subfloat[Input]{    \includegraphics[width=\mywidth]{figures/learning_optim/input.jpg}\label{fig:lo:in}}
        %  & \subfloat[GT]{    \includegraphics[width=\mywidth]{figures/learning_optim/gt.jpg}\label{fig:lo:gt}}
        %  &
        %  &
        %  \\
         \rotatebox{90}{\hspace{0mm}Learning}
         &
         &  \subfloat[CONet2D]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/ConvONet2D.jpg}\label{fig:lo:onet2}}
         &  \subfloat[CONet3D]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/ConvONet3D.jpg}\label{fig:lo:onet3}}
         &  \subfloat[SAP]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/SAP_learning.jpg}\label{fig:lo:sap}}
         &  \subfloat[DGNN]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/DGNN.jpg}\label{fig:lo:dgnn}}         
         &  \subfloat[POCO]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/POCO.jpg}\label{fig:lo:poco}}
         & \subfloat[Input]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/input.png}\label{fig:lo:in}}
         \\
         \rotatebox{90}{\hspace{-1mm}Optimization}
         & \subfloat[IGR]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/igr.jpg}\label{fig:lo:igr}}
         &  \subfloat[LIG]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/lig.jpg}\label{fig:lo:lig}}
         &  \subfloat[P2M]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/P2M.jpg}\label{fig:lo:p2m}}
         &  \subfloat[SAP\optim]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/SAP.jpg}\label{fig:lo:sap2}}
         &  \subfloat[SPSR]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/SPSR.jpg}\label{fig:lo:spsr}}         
         &  \subfloat[RESR]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/etal.jpg}\label{fig:lo:lab}}   
         & \subfloat[GT]{    \includegraphics[width=\mywidth,mytrim]{figures/learning_optim/gt.jpg}\label{fig:lo:gt}}
    \end{tabular}
\caption[Learning- vs. optimization-based reconstructions]{\textbf{Learning- vs. optimization-based reconstructions (E6):} We show reconstructions of \emph{dancing children} from Berger \etal from a low resolution input point cloud with noise (\subref{fig:lo:in}) and the ground truth shape (\subref{fig:lo:gt}). The methods used in the first row (\subref{fig:lo:onet2} - \subref{fig:lo:poco})  were trained on ShapeNet, on point clouds with the same sampling as the one used here. In the second row (\subref{fig:lo:igr} - \subref{fig:lo:spsr}) we show the reconstructions for the same shape (from the same sampling) from optimization-based methods.
}
    \label{fig:ch2:learning_optim}
\end{figure*}

==> figures/learning_results/iou_figure.tex <==
\begin{figure*}
	\centering\scriptsize 
	\definetrim{mytrim}{0 95 0 95}

\includegraphics[width=\textwidth]{figures/learning_results/iou_components_barplot.png}

	\caption[Volumetric \acl*{iou} and \acl*{noc} for learning-based reconstructions]{
		\textbf{Volumetric \acl*{iou} and \acl*{noc} for learning-based reconstructions:} 
		We show the mean volumetric \acl*{iou} of ground truth and reconstructed surfaces as well as the mean \acl*{noc} of the reconstructed surfaces for the learning experiments \hyperref[e1]{E1} to \hyperref[e5]{E5} for all methods. Except for \hyperref[e2]{E2}, at least one learning method (blue shading) has a higher volumetric \ac{iou} compared to the traditional methods (red shading). SPRS \cite{screened_poisson} is the only method that produces surfaces with a high volumetric \ac{iou} in each experiment. However, it also produces the least compact surfaces on average (\ie surfaces with the highest \ac{noc}).
	}
	\label{fig:ch2:learning_iou}
\end{figure*}

==> figures/setup/experiments_figure.tex <==
\begin{figure}

\captionsetup[sub]{labelfont=scriptsize,textfont=scriptsize,justification=centering}
    \centering
    \newcommand{\mywidth}{0.9\textwidth}

         \includegraphics[width=\mywidth]{figures/setup/experiments}
     

    \caption[Benchmark setup]{\textbf{Benchmark setup:}  
We show an overview of our experimental setup. In \hyperref[e1]{E1} to \hyperref[e4]{E4}, we train surface reconstruction methods on noisy point clouds of ShapeNet objects.  In \hyperref[e1]{E1}, we test on the ShapeNet test set. In \hyperref[e2]{E2}, we test on ShapeNet, but from denser point clouds with noise and outliers. In \hyperref[e3]{E3}, we test on the simpler ModelNet objects with the same sampling as in \hyperref[e1]{E1}. In \hyperref[e4]{E4}, we test on five Berger \etal shapes with the same sampling as in \hyperref[e1]{E1}. In \hyperref[e5]{E5}, we train the methods on the simpler ModelNet dataset and test on ShapeNet, both with the same sampling as in \hyperref[e1]{E1}. In \hyperref[e6]{E6}, we test optimization-based methods on synthetic range scans of the Berger \etal dataset.
}
    \label{ch2:fig:benchmark}
\end{figure}


==> figures/surface.tex <==
\tdplotsetmaincoords{60}{00} %
\centering
\begin{tabular}{cccc}

\begin{subfigure}{0.23\textwidth}
\resizebox{\linewidth}{.13\textheight}{\begin{tikzpicture}[tdplot_main_coords,
vertex/.style={fill=black, circle, text width = 1mm, inner sep=0pt},
]
    \node[vertex]  (p1) at (0,0,0) {};
    \node[vertex]  (p2) at (1,-1,0) {};
    \node[vertex]  (p3) at (1,1,0.2) {};
    \node[vertex]  (p4) at (2,0,0) {};
    %\node[fill=black, circle, text width = 1mm, inner sep=0pt]  (p5) at (3,0.5,0.2) {};


    \shade[ball color = gray!40, opacity = 0.4] (0.66,0,0.066) circle (0.7cm);
    \draw (0.66,0,0.066) circle (0.7cm);
    %\draw [dashed] (1.36,0,0.066) arc (0:360:0.7 and 0.3);


    \shade[ball color = gray!40, opacity = 0.4] (1.33,0,0.066) circle (0.7cm);
    \draw (1.33,0,0.066) circle (0.7cm);

    \draw [SURFCOLOR, thick, dashed] (p3) -- (p4) -- (p2);
    \draw [SURFCOLOR, thick] (p1) -- (p2) -- (p3) -- (p1);

    \draw [blue, ->] (p1) to [out=90,in=180] (1,2,0) to [out=0,in=90] (p4);
\end{tikzpicture}}
\caption{Advancing-Front.}
\label{fig:surface:a}
\end{subfigure}
&
\begin{subfigure}{0.23\textwidth}
\resizebox{\linewidth}{.13\textheight}{\begin{tikzpicture}[tdplot_main_coords,
svertex/.style={fill=black, circle, text width = 0.8mm, inner sep=0pt},
vertex/.style={fill=black, circle, text width = 1mm, inner sep=0pt},
network/.pic={
 \node[svertex] (n11) at (-1,0) {};
 \node[svertex] (n12) at (0,0) {};
 \node[svertex] (n13) at (1,0) {};
 \node[svertex] (n21) at (-1,-1) {};
 \node[svertex] (n22) at (0,-1) {};
 \node[svertex] (n23) at (1,-1) {};
 \node[svertex] (n32) at (0,-2) {};
 \draw[-] (n11) -- (n21) -- (n32) -- (n22) -- (n11) -- (n23) -- (n32);
 \draw[-] (n12) -- (n21) -- (n13) -- (n21);
 \draw[-] (n12) -- (n23) -- (n13);
 \draw[-] (n13) -- (n22);
\draw[->] (n32) -- (0,-3);
 }
]
    \node[vertex]  (p1) at (0,0,0) {};
    \node[vertex]  (p2) at (1,-1,0) {};
    \node[vertex]  (p3) at (1,1,0.2) {};
    \node[vertex]  (p4) at (2,0,0) {};
    %\node[fill=black, circle, text width = 1mm, inner sep=0pt]  (p5) at (3,0.5,0.2) {};

    \draw (1.8,1.4,0.1) pic[scale=0.3, rotate=-30] {network};

    \draw [SURFCOLOR, thick, dashed] (p3) -- (p4);
    \draw [SURFCOLOR, thick] (p1) -- (p2) -- (p3) -- (p1);

\end{tikzpicture}}
\caption{Selection-Based.}
\label{fig:surface:b}
\end{subfigure}
&
\begin{subfigure}{0.23\textwidth}
\resizebox{\linewidth}{.13\textheight}{\begin{tikzpicture}[tdplot_main_coords,
vertex/.style={fill=black, circle, text width = 1mm, inner sep=0pt},
]
    \node[vertex]  (p1) at (0,0,0) {};
    \node[vertex]  (p2) at (1,-1,0) {};
    \node[vertex]  (p3) at (1,1,0.2) {};
    \node[vertex]  (p4) at (2,0,0) {};

    \fill[opacity=0.2,blue] (-0.5,0,0.2) -- (0.5,2,0.2) -- (2.5,2,0.2) -- (1.5,0,0.2) -- cycle;

    \node[vertex, blue]  (p1p) at (0,0.5,0.2) {};
    \node[vertex, blue]  (p2p) at (1,0.3,0.2) {};
    \node[vertex, blue]  (p4p) at (2,1.2,0.2) {};

    \draw [->] (p1) -- (p1p);
    \draw [->] (p2) -- (p2p);
    \draw [->] (p4) -- (p4p);

     \draw[-, dashed, SURFCOLOR] (p1p) -- (p2p) -- (p3) -- (p1p);
     \draw[-, dashed, SURFCOLOR] (p3) -- (p4p) -- (p2p);

\end{tikzpicture}}
\caption{Projection-Based.}
\label{fig:surface:c}
\end{subfigure}
&
\begin{subfigure}{0.23\textwidth}
\resizebox{\linewidth}{.13\textheight}{\begin{tikzpicture}[tdplot_main_coords,
svertex/.style={fill=black, circle, text width = 0.8mm, inner sep=0pt},
vertex/.style={fill=black, circle, text width = 1mm, inner sep=0pt},
network/.pic={
 \node[svertex] (n11) at (-1,0) {};
 \node[svertex] (n12) at (0,0) {};
 \node[svertex] (n13) at (1,0) {};
 \node[svertex] (n21) at (-1,-1) {};
 \node[svertex] (n22) at (0,-1) {};
 \node[svertex] (n23) at (1,-1) {};
 \node[svertex] (n32) at (0,-2) {};
 \draw[-] (n11) -- (n21) -- (n32) -- (n22) -- (n11) -- (n23) -- (n32);
 \draw[-] (n12) -- (n21) -- (n13) -- (n21);
 \draw[-] (n12) -- (n23) -- (n13);
 \draw[-] (n13) -- (n22);
\draw[->] (n32) -- (0,-3);
 }
]
    \node[vertex]  (p1) at (0,0,0) {};
    \node[vertex]  (p2) at (1,-1,0) {};
    \node[vertex]  (p3) at (1,1,0.2) {};
    \node[vertex]  (p4) at (2,0,0) {};


    \node[vertex, blue]  (p1p) at (0.5,0.5,1.0) {};
    \node[vertex, blue]  (p2p) at (1.5,0.5,1.0) {};
    \node[vertex, blue]  (p3p) at (1.5,1.5,1.0) {};
    \node[vertex, blue]  (p4p) at (0.5,1.5,1.0) {};
        
    \fill[opacity=0.2,blue] (p1p.center) -- (p2p.center) -- (p3p.center) -- (p4p.center) -- (p1p.center);

    \draw[-, dashed, SURFCOLOR] (p1p) -- (p2p) -- (p3p) -- (p4p) -- (p1p) -- (p3p);
   
    
    \draw[->, blue] (p1p) -- ($(p1p)!0.7!(p1)$);
    \draw[->, blue] (p2p) -- ($(p2p)!0.7!(p3)$);
    \draw[->, blue] (p3p) -- ($(p3p)!0.7!(p4)$);
    \draw[->, blue] (p4p) -- ($(p4p)!0.7!(p2)$);

    \draw (-0.2,0,1) pic[scale=0.3, rotate=90] {network};
\end{tikzpicture}}
\caption{Deformation-Based.}
\label{fig:surface:d}
\end{subfigure}
\end{tabular}


==> figures/survey/ballpivot_figure.tex <==
\begin{figure}[h]
\tdplotsetmaincoords{60}{00}
  \begin{center}
    \resizebox{.5\linewidth}{.13\textheight}{\begin{tikzpicture}[tdplot_main_coords,
vertex/.style={fill=black, circle, text width = 1mm, inner sep=0pt},
]
    \node[vertex]  (p1) at (0,0,0) {};
    \node[vertex]  (p2) at (1,-1,0) {};
    \node[vertex]  (p3) at (1,1,0.2) {};
    \node[vertex]  (p4) at (2,0,0) {};

    \shade[ball color = gray!40, opacity = 0.4] (0.66,0,0.066) circle (0.7cm);
    \draw (0.66,0,0.066) circle (0.7cm);

    \shade[ball color = gray!40, opacity = 0.4] (1.33,0,0.066) circle (0.7cm);
    \draw (1.33,0,0.066) circle (0.7cm);

    \draw [SURFCOLOR, thick, dashed] (p3) -- (p4) -- (p2);
    \draw [SURFCOLOR, thick] (p1) -- (p2) -- (p3) -- (p1);

    \draw [blue, ->] (p1) to [out=90,in=180] (1,2,0) to [out=0,in=90] (p4);
\end{tikzpicture}}
  \end{center}
  \caption{Ball-Pivoting algorithm.}
  \label{fig:ball}
\end{figure}

==> figures/survey/projection_figure.tex <==
\begin{figure}[h]
\tdplotsetmaincoords{60}{00}
  \begin{center}
\resizebox{.5\linewidth}{.13\textheight}{\begin{tikzpicture}[tdplot_main_coords,
vertex/.style={fill=black, circle, text width = 1mm, inner sep=0pt},
]
    \node[vertex]  (p1) at (0,0,0) {};
    \node[vertex]  (p2) at (1,-1,0) {};
    \node[vertex]  (p3) at (1,1,0.2) {};
    \node[vertex]  (p4) at (2,0,0) {};

    \fill[opacity=0.2,blue] (-0.5,0,0.2) -- (0.5,2,0.2) -- (2.5,2,0.2) -- (1.5,0,0.2) -- cycle;

    \node[vertex, blue]  (p1p) at (0,0.5,0.2) {};
    \node[vertex, blue]  (p2p) at (1,0.3,0.2) {};
    \node[vertex, blue]  (p4p) at (2,1.2,0.2) {};

    \draw [->] (p1) -- (p1p);
    \draw [->] (p2) -- (p2p);
    \draw [->] (p4) -- (p4p);

     \draw[-, dashed, SURFCOLOR] (p1p) -- (p2p) -- (p3) -- (p1p);
     \draw[-, dashed, SURFCOLOR] (p3) -- (p4p) -- (p2p);

\end{tikzpicture}}
  \end{center}
  \caption{Projection-based methods.}
  \label{fig:surface:projection}
\end{figure}

==> sections/999_changes.tex <==
\begin{center}
\textbf{\LARGE
A Survey and Benchmark \\ of Automatic
Surface Reconstruction \\ from Point Clouds~\\~\\
\large Response to Reviewers.
~\\~\\}
\end{center}

We express our gratitude to the reviewers for their detailed and constructive feedback, which has significantly enhanced the quality of our manuscript. We also appreciate that our work has been described as comprehensive (\RONE, \RTWO, \RTHREE) interesting (\RONE), beneficial for the community (\RTWO, \RTHREE), insightful (\RTHREE), and clear (\RTHREE, \RFOUR).

\vspace{0.3cm}\noindent\textbf{Improved clarity (\RONE, \RTWO, \RTHREE, \RFOUR).} In response to the reviewers' suggestions, we have extensively revised the manuscript to improve clarity. Following \RONE's recommendation, the conclusions are now more prominently highlighted in both the abstract and the introduction, offering readers a clearer understanding of the paper's core contributions. Section 3 has been entirely rewritten for greater clarity and consistency when detailing various methods, and we have standardized our naming conventions and section titles throughout the paper. Additionally, as per \RFOUR's suggestion, we now include a comprehensive schematic representation of the methods (Figure 3), helping readers navigate this intricate field.

In fact, we have undertaken a comprehensive rewrite of the entirety of the paper to enhance its clarity. We recommend that the reviewers revisit Sections 3.2 and 4.2, where we have made the most significant improvements in terms of presentation.

\vspace{0.3cm}\noindent\textbf{Improved and additional figures (\RONE, \RTWO).}
All figures have been revised to enhance their consistency and clarity. Specifically, Figure 2 has undergone significant improvement. Responding to \RTWO's input, we introduced a new figure (Figure 3) illustrating the principal surface reconstruction approaches and removed the table with qualitative assessments of method performance.

\vspace{0.3cm}\noindent\textbf{Additional references and methods (\RONE, \RTWO).} 
{We have updated Sections 2, 3 and 4 with novel state-of-the-art references.} We have incorporated all the references recommended by the reviewers, notably including \acl{nksr}. Unfortunately, due to implementation issues, we could not retrain this method for inclusion in our benchmark.

\vspace{0.3cm}\noindent\textbf{Limitations (\RONE, \RTHREE, \RFOUR).} We added a new section on limitations, discussing our decision to exclude NERF-type methods and addressing the limitations of our synthetic MVS scanning procedure.

\vspace{0.3cm}\noindent\textbf{Merging Experiments (\RTWO).} As suggested, we have merged experiment E4 (learning-based methods on Berger's shapes) and experiment E7 (learning \textit{vs} optimization on Berger's shapes) to streamline the benchmark.
We acknowledge the suggestion to include the optimization-based methods directly in the experiments E1-E4 instead of presenting the additional experiment E6 to compare learning- and optimization-based methods. However, the tested neural-network-based optimization methods are particularly slow compared to pre-trained learning models or traditional methods, and take several minutes to reconstruct each shape. As the test sets of E1-E4 comprise several thousands of distinct shapes, adding optimization methods to all experiments would take months of uninterrupted computation. On the other hand, we took advantage of the speed of learning-based methods to evaluate them on large test sets.

\vspace{0.3cm}\noindent\textbf{Normal Error Metric (\RTWO).} 
In the field of photogrammetry, angular error is commonly employed to assess normal consistency. However, within the learning-based surface reconstruction community, the cosine distance is the predominant measure. We have opted to align with the latter approach, as it offers greater discriminative power for smaller errors.

\vspace{0.3cm}\noindent\textbf{Scanning procedure (\RONE).}
We acknowledge that our approach to simulating \ac{mvs} scanning may not perfectly mirror real-world acquisitions characteristics. The necessity for ground truth meshes to train and evaluate methods in our benchmark makes it challenging to work with actual \ac{mvs} scans due to various practical difficulties. Even extensive LiDAR acquisitions, which are both costly and time-intensive, often fall short of producing complete surfaces owing to inherent self-occlusion issues. Our generation of \ac{mvs} point clouds, varying in density and outlier ratios, aims to encompass a wide spectrum of \ac{mvs} pipeline outputs, albeit within the limitations of our synthetic setup.
For range scanning we use the method of Berger~\etal which is published as a peer-reviewed method like Blensor.

\vspace{0.3cm}\noindent\textbf{Categorization of methods (\RTWO).} We have rethought our categorization of methods and now group them according to their dependence on a training set. We also acknowledge the hybrid nature of LIG.


\vfill

==> tables/all_learning_bk.tex <==
\begin{table*}
\caption[Numerical results for learning-based reconstructions]{\textbf{Numerical results for learning-based reconstructions (\hyperref[e1]{E1} to \hyperref[e5]{E5})}:
\LOIC{
$^\star$ non deep-learning methods.
}

\acs*{spsr} \cite{screened_poisson} is the only method that reconstructs surfaces with a high volumetric \acf*{iou} and a low \acf*{cd} in each experiment. Therefore, its reconstructions have the highest mean volumetric \ac*{iou} and the lowest mean \ac*{cd}. However, \acs*{spsr} also reconstructs the least compact surfaces on average (\ie surfaces with the highest \acl*{noc}). Labatut \etal \cite{Labatut2009a} reconstructs the most compact surfaces. 
The reconstructions of \ac*{dgnn} \cite{dgnn} have the highest mean volumetric \ac*{iou} of the tested learning methods. 
The reconstructions of \ac*{sap} \cite{Peng2021SAP} have the lowest mean \ac*{cd} of the tested learning methods and the highest normal consistency. \Ac*{conet} and \ac*{spsr} are the only methods that reconstruct surfaces without boundary and non-manifold edges.
}
\centering
\resizebox{\textwidth}{!}{

\begin{tabular}{l@{~}rcccccc|cccccc}
\toprule
& & \multicolumn{6}{c|}{\textbf{Volumetric IoU} (\%)~~[$\uparrow$]}
& \multicolumn{6}{c}{\textbf{Normal consistency} (\%)~~[$\uparrow$]}
\\
\textbf{Method} &                &            E1 &            E2 &            E3 &            E4 &            E5 &          Mean &            E1 &            E2 &            E3 &            E4 &            E5 &          Mean \\
\midrule
\textbf{ConvONet2D   } &          \cite{Peng2020} &            85.0 &          47.3 &          79.3 &          65.1 &          68.3 &            69 &          92.7 &          76.4 &            90 &            78 &        87.8 &            85 \\
\textbf{ConvONet3D   } &          \cite{Peng2020} &          84.8 &          15.1 &          83.6 &          76.4 &            51.0 &          62.2 &            93 &          71.8 &          93.1 &          87.2 &        82.5 &          85.5 \\
\textbf{SAP          } &       \cite{Peng2021SAP} &          88.7 &          59.8 &          89.2 &          78.3 &          54.9 &          74.2 &          93.5 & \textbf{86.7} &          94.1 &            89 &        87.1 & \textbf{90.1} \\
\textbf{DGNN         } &              \cite{dgnn} &          84.5 &          38.1 &            87.0 &          82.9 & \textbf{84.4} &          75.4 &          85.4 &          68.8 &          88.5 &          85.2 &        85.5 &          82.7 \\
\textbf{POCO         } &    \cite{boulch2022poco} & \textbf{89.5} &          8.74 & \textbf{90.6} & \textbf{83.9} &          40.9 &          62.7 & \textbf{93.6} &          75.6 & \textbf{94.2} & \textbf{89.5} &        82.9 &          87.1 \\
\textbf{SPSR         } &  \cite{screened_poisson} &          77.1 & \textbf{80.7} &          80.7 &          77.6 &          74.6 & \textbf{78.1} &          87.7 &          83.2 &          89.1 &          86.3 & \textbf{88} &          86.9 \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} &          80.3 &          60.4 &          83.9 &          79.4 &          80.3 &          76.9 &            81.0 &            73 &          84.6 &          80.8 &          81.0 &          80.1 \\
\midrule
& & \multicolumn{6}{c|}{\textbf{Chamfer distance} (per-point ave. \%) ~~[$\downarrow$]}
& \multicolumn{6}{c}{\textbf{Number of components} ~~[$\downarrow$]}
\\
\textbf{Method} &  &             E1 &             E2 &             E3 &             E4 &             E5 &           Mean &            E1 &            E2 &            E3 &         E4 &            E5 &         Mean \\
\midrule
\textbf{ConvONet2D   } &          \cite{Peng2020} &          0.553 &           7.51 &          0.997 &           1.43 &         0.979 &           2.29 &           1.6 &          34.8 &          2.55 &        3.6 &           3.2 &         9.16 \\
\textbf{ConvONet3D   } &          \cite{Peng2020} &          0.546 &           10.9 &           0.76 &          0.887 &          2.44 &            3.1 &          1.37 &          13.6 &           1.6 &        2.6 &           1.5 &         4.13 \\
\textbf{SAP          } &       \cite{Peng2021SAP} &          0.437 &           2.09 &          0.547 &          0.734 &         0.924 &          0.946 &          2.71 &            86 &          3.45 &        5.6 &          10.5 &         21.7 \\
\textbf{DGNN         } &              \cite{dgnn} &          0.549 &           2.54 &          0.635 &          0.586 & \textbf{0.55} &          0.973 &          1.31 &          16.1 &          1.13 & \textbf{1} &          1.31 &         4.16 \\
\textbf{POCO         } &    \cite{boulch2022poco} & \textbf{0.416} &           10.5 & \textbf{0.516} & \textbf{0.579} &          1.32 &           2.67 &          2.32 &           178 &          2.82 &          2 &          16.3 &         40.2 \\
\textbf{SPSR         } &  \cite{screened_poisson} &          0.801 & \textbf{0.659} &          0.873 &          0.786 &         0.886 & \textbf{0.801} &          9.26 &           185 &          11.1 &          8 &          3.24 &         43.3 \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} &          0.665 &           6.97 &          0.747 &          0.671 &         0.665 &           1.94 & \textbf{1.22} & \textbf{9.02} & \textbf{1.05} & \textbf{1} & \textbf{1.22} & \textbf{2.7} \\
\midrule
& & \multicolumn{6}{c|}{\textbf{Number of boundary edges} ~~[$\downarrow$]}
& \multicolumn{6}{c}{\textbf{Number of non-manifold edges}~~[$\downarrow$]}
\\
\textbf{Method} &        &         E1 &         E2 &         E3 &         E4 &         E5 &       Mean &         E1 &         E2 &         E3 &         E4 &         E5 &       Mean \\
\midrule
\textbf{ConvONet2D   } &          \cite{Peng2020} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{ConvONet3D   } &          \cite{Peng2020} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{SAP          } &       \cite{Peng2021SAP} & \textbf{0} &    0.00923 & \textbf{0} & \textbf{0} &       8.44 &       1.69 & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{DGNN         } &              \cite{dgnn} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} &       1.35 &       2.24 &      0.646 &        0.4 &       1.69 &       1.26 \\
\textbf{POCO         } &    \cite{boulch2022poco} & \textbf{0} &        121 & \textbf{0} & \textbf{0} &       41.7 &       32.5 & \textbf{0} &    0.00154 & \textbf{0} & \textbf{0} & \textbf{0} &   0.000308 \\
\textbf{SPSR         } &  \cite{screened_poisson} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} &       9.35 &       28.5 &       8.47 &        9.6 &       9.35 &       13.1 \\
\bottomrule
\end{tabular}


}
\label{tab:all_learning_experiments}
\end{table*}

==> tables/all_optim_bk.tex <==
\begin{table*}
\caption[Numerical results for optimization-based reconstructions]{\textbf{Numerical results for optimization-based reconstructions (\hyperref[e6]{E6})}: LR is a low resolution scan, HR a high resolution scan, HRN a high resolution scan with noise, HRO a high resolution scan with outliers, and HRNO a high resolution scan with noise and outliers. The methods are optimized per shape and per scan using standard settings as mentioned in the corresponding publications. The traditional method of Labatut~\etal~\cite{Labatut2009a} reconstructs the surfaces with the highest mean volumetric \acl*{iou} and lowest mean \acl*{cd}.}
\centering
\resizebox{\textwidth}{!}{

\begin{tabular}{l@{~}rcccccc|cccccc}
\toprule
& & \multicolumn{6}{c|}{\textbf{Volumetric IoU} (\%)~~[$\uparrow$]}
& \multicolumn{6}{c}{\textbf{Normal consistency} (\%)~~[$\uparrow$]}
\\
\textbf{Method} &                                   &            LR &            HR &            HRN &            HRO &            HRNO &          Mean &            LR &            HR &            HRN &            HRO &            HRNO &          Mean \\
\midrule
\textbf{IGR          } &         \cite{Gropp2020} &          80.8 &          92.5 & \textbf{83.6} &          63.7 &          62.7 &          76.7 &            88 & \textbf{96.3} &        83.9 &          77.8 &          71.5 &          83.5 \\
\textbf{LIG          } &               \cite{lig} &          46.9 &          50.3 &          63.9 &            66 &          63.8 &          58.2 & \textbf{88.7} &          92.2 & \textbf{89} &            77 &          75.2 &          84.4 \\
\textbf{P2M          } &        \cite{point2mesh} &          75.2 &          83.3 &          75.5 &          71.3 &          67.8 &          74.6 &          86.3 &          92.2 &        88.1 &          84.5 &          82.1 &          86.6 \\
\textbf{SAP          } &       \cite{Peng2021SAP} &          75.6 &          89.1 &          72.4 &          55.3 &          34.9 &          65.4 &          83.4 &          94.8 &        61.6 &          74.5 &          55.3 &          73.9 \\
\textbf{SPSR         } &  \cite{screened_poisson} &          77.7 &          90.2 &          82.8 &          90.3 & \textbf{82.1} &          84.6 &          88.1 &            96 &        88.1 & \textbf{96.2} & \textbf{85.8} & \textbf{90.9} \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} & \textbf{81.3} & \textbf{93.4} &          80.1 & \textbf{93.4} &          79.1 & \textbf{85.5} &          87.6 &            96 &        66.3 &          94.9 &          66.5 &          82.3 \\
\midrule
& & \multicolumn{6}{c|}{\textbf{Chamfer distance} (per-point ave. \%) ~~[$\downarrow$]}
& \multicolumn{6}{c}{\textbf{Number of components} ~~[$\downarrow$]}
\\
\textbf{Method} &                               &             LR &            HR &            HRN &            HRO &            HRNO &           Mean &            LR &            HR &            HRN &            HRO &            HRNO &         Mean \\
\midrule
\textbf{IGR          } &         \cite{Gropp2020} &          0.674 &          0.322 & \textbf{0.554} &           7.96 &           7.72 &           3.45 &          6.8 & \textbf{1.2} &         35.2 &           44 &       97.4 &          36.9 \\
\textbf{LIG          } &               \cite{lig} &          0.745 &          0.581 &          0.781 &           7.89 &            7.8 &           3.56 &   \textbf{1} &   \textbf{1} &   \textbf{1} &          1.6 & \textbf{1} &          1.12 \\
\textbf{P2M          } &        \cite{point2mesh} &          0.817 &          0.473 &          0.729 &           1.53 &           2.13 &           1.13 & \textbf{1.2} &   \textbf{1} & \textbf{1.2} &          1.4 &        1.6 &          1.28 \\
\textbf{SAP          } &       \cite{Peng2021SAP} &          0.852 &           0.32 &          0.701 &           3.99 &           3.93 &           1.96 &         73.2 &         85.6 &          937 &      1.8e+03 &   1.96e+03 &           971 \\
\textbf{SPSR         } &  \cite{screened_poisson} &          0.794 &          0.369 &          0.572 &          0.362 & \textbf{0.607} &          0.541 & \textbf{1.2} &          1.6 &          3.6 &          3.8 &       20.2 &          6.08 \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} & \textbf{0.635} & \textbf{0.314} &          0.608 & \textbf{0.339} &          0.641 & \textbf{0.507} &   \textbf{1} &   \textbf{1} & \textbf{1.2} & \textbf{1.2} & \textbf{1} & \textbf{1.08} \\
\midrule
& & \multicolumn{6}{c|}{\textbf{Number of boundary edges} ~~[$\downarrow$]}
& \multicolumn{6}{c}{\textbf{Number of non-manifold edges}~~[$\downarrow$]}
\\
\textbf{Method} &        &         LR &            HR &            HRN &            HRO &            HRNO &       Mean &         LR &            HR &            HRN &            HRO &            HRNO &       Mean \\
\midrule
\textbf{IGR          } &         \cite{Gropp2020} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} &        0.8 &        0.8 &        5.2 &        4.2 &        2.2 \\
\textbf{LIG          } &               \cite{lig} &         69 &       42.8 &       17.2 & \textbf{0} & \textbf{0} &       25.8 & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{P2M          } &        \cite{point2mesh} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{SAP          } &       \cite{Peng2021SAP} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} &        449 &       89.8 & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{SPSR         } &  \cite{screened_poisson} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} &          1 &        5.8 &       24.4 &        3.8 &         22 &       11.4 \\
\bottomrule
\end{tabular}


}
\label{tab:all_optim_experiments}
\end{table*}

==> tables/berger_confs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}
\centering
\caption[Scanning configurations for Berger \etal benchmark]{\textbf{Scanning configurations for Berger \etal benchmark:} We show the five different scanner configurations used in our modified version of the Berger et al.'s scanning procedure. We use the resulting scans to evaluate object-level reconstruction with varying point-cloud defects and for training data generation. For the low resolution (LR) scans the scanning process results in $1000$ to $3000$ points per shape, and for the high resolution (HR), the scanning process yields around $10\,000$ to $30\,000$ points.}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{l}{} & \textbf{Low res. (LR)} & \textbf{High res. (HR)} & \textbf{HR + noise (HRN)} & \textbf{HR + outliers (HRO)} & \textbf{HR + noise + outliers (HRNO)} \\ \midrule
Camera resolution x, y & 50, 50 & 100, 100 & 100, 100 & 100, 100 & 100, 100 \\
Scanner positions & 5 & 10 & 10 & 10 & 10 \\
Min/max range & 70/300 & 70/300 & 70/300 & 70/300 & 70/300 \\
Additive noise & 0 & 0 & 0.5 & 0 & 0.5 \\
Outliers (\%) & 0 & 0 & 0 & 0.1 & 0.1 \\ \bottomrule
\end{tabular}%
}
\label{tab:berger_confs}
\end{table*}

==> tables/conclusion_bk.tex <==
\begin{table*}
\caption[Summary of benchmark results]{\textbf{Summary:} 
We report the performance of all methods of our benchmark based on various qualitative criteria: $***$ good, $**$:fair, $*$: poor.
The traditional methods \ac{spsr}~\cite{screened_poisson} and Labatut~\etal~\cite{Labatut2009a} are the most versatile  tested in our benchmark.}
\label{tab:conclusion}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lrcccccccc@{}}
\toprule
&& \multicolumn{4}{l}{\textbf{Robustness to out-of-distribution}}                                   & \multicolumn{3}{l}{\textbf{Mesh quality}}                                                                 & \multicolumn{1}{l}{\textbf{Runtime}} 
\\ \midrule
\emph{\textbf{Learning}}  &
& noise & outliers & density     & category & watertightness & manifoldness & compactness & w/o training        \\
\cmidrule{1-2} 
ConvONet2D&          \cite{Peng2020}                  & *                         & *                            & *                               & *                            & ***                                & ***                              & *                               & ***                 \\
ConvONet3D&          \cite{Peng2020}                  & *                         & *                            & *                               & *                            & ***                                & ***                              & ***                             & ***                 \\
SAP&       \cite{Peng2021SAP}                         & **                        & **                           & **                              & **                            & ***                                 & ***                              & *                               & ***                 \\
DGNN&              \cite{dgnn}                        & *                         & *                            & *                               & ***                           & ***                                & **                               & ***                             & ***                 \\
POCO&    \cite{boulch2022poco}                        & **                        & *                            & *                               & **                            & ***                                 & ***                              & *                               & **            \\ \midrule
&& \multicolumn{4}{l}{\textbf{Robustness to}}                                                                & \multicolumn{3}{l}{\textbf{Mesh quality}}                                                                  & \multicolumn{1}{l}{\textbf{Runtime}}               
\\ \midrule
\emph{\textbf{Optimization}}   &
& noise & outliers & low density & category & watertightness & manifoldness & compactness & w/ training         \\
\cmidrule{1-2}
IGR&         \cite{Gropp2020}                         & ***                       & **                           & **                              & ***                          & ***                                & **                               & *                               & *                   \\
LIG&               \cite{lig}                         & *                         & *                            & *                               & ***                          & **                                  & ***                              & ***                             & *                   \\
P2M&        \cite{point2mesh}                         & *                         & **                           & *                               & ***                          & ***                                & ***                              & ***                             & *                   \\
SAP&       \cite{Peng2021SAP}                         & *                         & *                            & *                               & ***                          & ***                                 & ***                              & *                               & *                   \\
SPSR&  \cite{screened_poisson}                        & ***                       & ***                          & ***                             & ***                          & ***                                & ***                              & *                               & ***                 \\
Labatut~\etal&      \cite{Labatut2009a}                     & ***                       & ***                          & ***                             & ***                          & ***                                & *                                & ***                             & ***                 \\ \bottomrule
\end{tabular}
}
\end{table*}


==> tables/conclusion_table.tex <==
\begin{table*}
\caption[Summary of benchmark results]{\textbf{Summary:} 
We report the performance of all methods of our benchmark based on various qualitative criteria with the following grades: $***$ good, $**$:fair, $*$: poor.
The traditional methods \ac{spsr}~\cite{screened_poisson} and Labatut~\etal~\cite{Labatut2009a} are the most versatile  tested in our benchmark.}
\label{tab:conclusion}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}llrcccccccc@{}}
\toprule
&&& \multicolumn{4}{l}{\textbf{Robustness to out-of-distribution}}                                   & \multicolumn{3}{l}{\textbf{Mesh quality}}                                                                 & \multicolumn{1}{l}{\textbf{Runtime}} 
\\ \midrule

& &
& noise & outliers & density     & category & watertightness & manifoldness & compactness & w/o training        \\
\multirow{5}{*}{
\rotatebox{90}{\textbf{Learning}}} &ConvONet2D&          \cite{Peng2020}                  & *                         & *                            & *                               & *                            & ***                                & ***                              & *                               & ***                 \\
&\rowcolor{gray!10}ConvONet3D&          \cite{Peng2020}                  & *                         & *                            & *                               & *                            & ***                                & ***                              & ***                             & ***                 \\
&SAP&       \cite{Peng2021SAP}                         & **                        & **                           & **                              & **                            & ***                                 & ***                              & *                               & ***                 \\
&\rowcolor{gray!10}DGNN&              \cite{dgnn}                        & *                         & *                            & *                               & ***                           & ***                                & **                               & ***                             & ***                 \\
&POCO&    \cite{boulch2022poco}                        & **                        & *                            & *                               & **                            & ***                                 & ***                              & *                               & **            \\ \midrule
&&& \multicolumn{4}{l}{\textbf{Robustness to}}                                                                & \multicolumn{3}{l}{\textbf{Mesh quality}}                                                                  & \multicolumn{1}{l}{\textbf{Runtime}}               
\\ \midrule
&
&& noise & outliers & low density & category & watertightness & manifoldness & compactness & w/ training         \\
\multirow{6}{*}{
\rotatebox{90}{\textbf{Optimization}}}
&IGR&         \cite{Gropp2020}                         & ***                       & **                           & **                              & ***                          & ***                                & **                               & *                               & *                   \\
&\rowcolor{gray!10}LIG&               \cite{lig}                         & *                         & *                            & *                               & ***                          & **                                  & ***                              & ***                             & *                   \\
&P2M&        \cite{point2mesh}                         & *                         & **                           & *                               & ***                          & ***                                & ***                              & ***                             & *                   \\
&\rowcolor{gray!10}SAP&       \cite{Peng2021SAP}                         & *                         & *                            & *                               & ***                          & ***                                 & ***                              & *                               & *                   \\
&SPSR&  \cite{screened_poisson}                        & ***                       & ***                          & ***                             & ***                          & ***                                & ***                              & *                               & ***                 \\
&\rowcolor{gray!10}Labatut~\etal&      \cite{Labatut2009a}                     & ***                       & ***                          & ***                             & ***                          & ***                                & *                                & ***                             & ***                 \\ \bottomrule
\end{tabular}
}
\end{table*}


==> tables/experiments_table.tex <==
\begin{table*}
\caption[Benchmark setup]{
	\textbf{Benchmark setup:} 
We show an overview of our experimental setup. In E1 to E4, we train surface reconstruction methods on noisy point clouds of ShapeNet.  In E1, we test on the ShapeNet test set. In E2, we test on ShapeNet, but from denser point clouds with noise and outliers. In E3, we test on the simpler ModelNet objects with the same sampling as in E1. In E4, we train the methods on the simpler ModelNet dataset and test on ShapeNet, both with the same sampling as in E1. In E5, we test optimization-based methods on synthetic range scans of the Berger \etal dataset. And finally, in E6, we compare learning- and optimization-based methods on the same dataset (synthetic MVS scans of the Berger \etal dataset).
}
\begin{adjustbox}{max width=\textwidth}
\footnotesize
\centering
\begin{tabular}{ccccccccccccc}
\toprule
            & \multicolumn{6}{c}{\textbf{\textit{Training set}}}        &  \multicolumn{6}{c}{\textbf{\textit{Test set}}}                                         \\
\textbf{Experiment}  & \textbf{Name}          & \textbf{\#~shapes} & \textbf{complexity}    & \textbf{\#~points} &       \textbf{$\sigma$~noise} & \textbf{\%~outliers}    & \textbf{Name}    & \textbf{\#~shapes} & \textbf{complexity}    & \textbf{\#~points} & \textbf{$\sigma$~noise} & \textbf{\%~outliers}   \\ \midrule
1           & ShapeNet      & $30,661$  & $\star\star$  & $3,000$           & $0.005$       & $0$               & ShapeNet      & $1,300$   & $\star\star$  & $3,000$   & $0.005$       & $0$           \\
2           & ShapeNet      & $30,661$  & $\star\star$  & $3,000$           & $0.005$       & $0$               & ShapeNet      & $1,300$   & $\star\star$  & $10k$  & $0.005$       & $10$          \\
3           & ShapeNet      & $30,661$  & $\star\star$  & $3,000$           & $0.005$       & $0$               & ModelNet      & $506$     & $\star$       & $3,000$   & $0.005$       & $0$           \\
% 4           & ShapeNet      & $30,661$  & $\star\star$  & $3,000$           & $0.005$       & $0$               & Berger~\etal  & $5$       & $\star\star$  & $3,000$   & $0.005$       & $0$           \\
4           & ModelNet      & $3,979$   & $\star$       & $3,000$           & $0.005$       & $0$               & ShapeNet      & $1,300$   & $\star\star$  & $3,000$   & $0.005$       & $0$           \\ 
% 6           & SRD           & $3,979$   & $\star\star\star$& $500-50k$      & $0.000-0.025$ & $0-50$            & ETH3D         & $1,300$   & $\star\star$  & $3,000$   & $0.005$       & $0$           \\
\midrule
5           & \multicolumn{6}{c}{--}                                                           & Berger~\etal  & $5$       & $\star\star$  &\multicolumn{3}{c}{see \tabref{tab:berger_confs}} \\
\midrule
6           &  ShapeNet      & $30,661$  & $\star\star$  & $3,000$           & $0.005$       & $0$   & Berger~\etal  & $5$       & $\star\star$  & $3,000$   & $0.005$       & $0$                   \\
\midrule
7           &  ShapeNet      & $30,661$  & $\star\star$  & $3,000$           & $0.005$       & $0$   & Real  & $3$       & $\star\star\star$  & $10,000$   & \emph{variable}       & \emph{variable}                   \\
\bottomrule
% 5           & FamousThingi  & $50$      & $\star\star$  & $300$-$30,000$    & $0.005$       & $0$               & Berger~\etal  & $1,300$   & $10,000$  & $0.005$       & $10$          \\ \bottomrule
% 6           & FamousThingi  & $50$      & $\star\star$  & $300$-$30,000$    & $0.005$       & $0$               & ETH3D         & $3$       & $10,000$  & $0.005$       & $10$          \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{ch2:tab:benchmark_supp}
\end{table*}



==> tables/learning_optim_bk.tex <==
\begin{table*}
\caption[Numerical results for learning- and optimization-based reconstructions]{\textbf{Numerical results for learning- and optimization-based reconstructions (\hyperref[e7]{E7})}: Learning- and optimization-based reconstruction of the Berger \etal test shapes from synthetic MVS scans. The learning methods were trained on synthetic MVS scans from ShapeNet. Optimization-based methods are optimized per scan using standard settings. BE stands for boundary edges and NME for non-manifold edges. Only the learning-based methods \ac{poco} and \ac{dgnn} reconstruct surfaces with a higher mean volumetric \acl*{iou} and lower mean \acl*{cd} than all optimization-based methods.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{}rcccccc}
% \toprule
\textbf{Method} &   
% &  \rot{\textbf{Vol. IoU} (\%)~~[$\uparrow$]} 
% & \rot{\textbf{Normal consistency} (\%)~~[$\uparrow$]} 
% & \rot{\textbf{Chamfer dist.} (per-point ave. \%) ~~[$\downarrow$]}
% &\rot{\textbf{N. of components} ~~[$\downarrow$]}
% &\rot{\textbf{N. of boundary edges} ~~[$\downarrow$]}
% &\rot{\textbf{N. of non-manifold edges}~~[$\downarrow$]}\\
&  \textbf{Vol. IoU} (\%) ~~[$\uparrow$]
& \textbf{Normal consist.} (\%) ~~[$\uparrow$] 
& \textbf{Chamfer dist.} ($\times 10^3$) ~~[$\downarrow$]
&\textbf{Components} ~~[$\downarrow$]
&\textbf{BE} ~~[$\downarrow$]
&\textbf{NME}~~[$\downarrow$]\\
\midrule
\emph{\textbf{Learning}}&&&&&&&\\
\cmidrule{1-2}
\textbf{ConvONet2D   } &          \cite{Peng2020} &          65.1 &            78 &           1.43 &        3.6 & \textbf{0} & \textbf{0} \\
\textbf{ConvONet3D   } &          \cite{Peng2020} &          76.4 &          87.2 &          0.887 &        2.6 & \textbf{0} & \textbf{0} \\
\textbf{SAP          } &       \cite{Peng2021SAP} &          78.3 &            89 &          0.734 &        5.6 & \textbf{0} & \textbf{0} \\
\textbf{DGNN         } &              \cite{dgnn} &          82.9 &          85.2 &          0.586 & \textbf{1} & \textbf{0} &        0.4 \\
\textbf{POCO         } &    \cite{boulch2022poco} & \textbf{83.9} & \textbf{89.5} & \textbf{0.579} &          2 & \textbf{0} & \textbf{0} \\
\midrule
\emph{\textbf{Optimization}}&&&&&&&\\
\cmidrule{1-2}
\textbf{IGR          } &         \cite{Gropp2020} &          78.3 &          83.8 &          0.775 &       15.4 & \textbf{0} &        0.4 \\
\textbf{LIG          } &               \cite{lig} &          45.7 &  		 86.6 &          0.831 & \textbf{1} &       65.6 & \textbf{0} \\
\textbf{P2M          } &        \cite{point2mesh} &          74.5 &            85 &          0.768 &          2 & \textbf{0} & \textbf{0} \\
\textbf{SAP          } &       \cite{Peng2021SAP} &          71.9 &            77 &          0.811 &        133 & \textbf{0} & \textbf{0} \\
\textbf{SPSR         } &  \cite{screened_poisson} &          77.6 &          86.4 &          0.785 &          8 & \textbf{0} & \textbf{0} \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} & 		 79.4 &          80.8 &          0.671 & \textbf{1} & \textbf{0} &        9.6 \\
\bottomrule
\end{tabular}


}
\label{tab:learning_optim_experiments}
\end{table*}

==> tables/survey.tex <==
\begin{table}
\caption[Overview of surface- and volume-based surface reconstruction methods]{\textbf{Overview of surface- and volume-based surface reconstruction methods:} We show an overview of surface- and volume-based surface reconstruction methods, both non-learning and learning-based, together with their input requirements (\emph{normals}, \emph{sensor pose}) and output type (\emph{triangle mesh} or \emph{implicit field}). Attributes denoted in brackets are optional.
% RF stands for receptive field. 
Methods with a \emph{local} receptive field divide the point cloud into smaller sub-regions 
% (\eg based on local neighborhoods) 
and define individual functions or surface patches for each sub-region. Methods with a \emph{global} receptive field
% do not fit locally independent functions or surface patches within the domain of the point cloud, but 
consider the entire point cloud at once. Methods denoted with \emph{both} combine local and global receptive fields. We test methods in \textbf{bold} in our benchmark.}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l@{}r@{}c@{}c@{}c@{}c@{}c@{}}
% \toprule
\textbf{Method}        &                     & \rotatebox[origin=l]{45}{learning}       & \rotatebox[origin=l]{45}{normals} & \rotatebox[origin=l]{45}{sensor pose} &  \rotatebox[origin=l]{45}{receptive field} & \rotatebox[origin=l]{45}{output}\\
\midrule
\emph{\textbf{Surface-based}}&&&&&\\
\cmidrule{1-2}
BPA           &\cite{bernardini1999ball} &             &	           &                 &local & triangle mesh \\
Sharf \etal   &\cite{sharf2006competing} &             &               &                 &both  & triangle mesh \\         
AtlasNet      &\cite{Groueix2018}        &  \checkmark &	           &                 &local & triangle mesh \\
IER           &        \cite{liu2020ier} &  \checkmark &	            &                & both & triangle mesh \\
PointTriNet   &        \cite{PointTriNet}&  \checkmark &	          &                  &local &  triangle mesh \\
DSE           &\cite{rakotosaona2021dse} &  \checkmark &	           &                 & local&triangle mesh \\
\textbf{P2M}  &        \cite{point2mesh} &             &              &                  & both &triangle mesh \\
\midrule
\emph{\textbf{Volume-based}}&&&&&\\
\cmidrule{1-2}
\textbf{SPSR         } &  \cite{screened_poisson} &               & \checkmark &                  &   both& implicit field \\
\textbf{Labatut~\etal} &      \cite{Labatut2009a} &             &             &\checkmark         &global &triangle mesh \\
ONet                   &      \cite{Mescheder2019}& \checkmark  &             &                   &global & implicit field  \\
DeepSDF                &      \cite{Park2019}     & \checkmark  &             &                   &global &implicit field  \\
IM-Net                 &            \cite{IM-Net} & \checkmark  &             &                   &global & implicit field  \\
\textbf{ConvONet   }   &          \cite{Peng2020} & \checkmark  &               &                 &  both & implicit field  \\
\textbf{IGR          } &         \cite{Gropp2020} & (\checkmark)& (\checkmark)&                   &global & implicit field  \\
\textbf{LIG          } &               \cite{lig} & \checkmark  &   \checkmark &                  & local &  implicit field  \\
\textbf{DGNN         } &              \cite{dgnn} &  \checkmark &               & \checkmark      & both & triangle mesh  \\
\textbf{SAP          } &       \cite{Peng2021SAP} & \checkmark  &               &                 &  both & implicit field  \\
P2S           &       \cite{points2surf} & \checkmark  &               &                 &  both & implicit field \\
\textbf{SAP          } &       \cite{Peng2021SAP} & (\checkmark)&               &                 &  both & implicit field \\
\textbf{POCO         } &    \cite{boulch2022poco} &  \checkmark &   (\checkmark)&                 &  local& implicit field \\
\bottomrule
\end{tabular}
}
\label{tab:survey}
\end{table}
